Influence maximization in unknown social networks: Learning Policies for Effective Graph Sampling

A serious challenge when finding influential actors in real-world social networks is the lack of knowledge about the structure of the underlying network. Current state-of-the-art methods rely on hand-crafted sampling algorithms; these methods sample nodes and their neighbours in a carefully constructed order and choose opinion leaders from this discovered network to maximize influence spread in the (unknown) complete network. In this work, we propose a reinforcement learning framework for network discovery that automatically learns useful node and graph representations that encode important structural properties of the network. At training time, the method identifies portions of the network such that the nodes selected from this sampled subgraph can effectively influence nodes in the complete network. The realization of such transferable network structure based adaptable policies is attributed to the meticulous design of the framework that encodes relevant node and graph signatures driven by an appropriate reward scheme. We experiment with real-world social networks from four different domains and show that the policies learned by our RL agent provide a 10-36% improvement over the current state-of-the-art method.

==> ablation_studies.tex <==
\section{Ablation Studies}
\label{sec:abl}
From the discussion is Section \ref{sec:rep}, we note that the important neural architecture components that were essential in encoding the network structure and node properties are Deepwalk embeddings and Differential pooling layers.
We also added step-rewards (see Section \ref{sec:mdpf}) to encourage the agent to discover larger graphs.

In this section, we investigate the importance of each of these components for training the model.
We consider three variants of our model. In the first variant, we don't provide step rewards. In the second variant, we use sum pooling rather that differential pooling layer. In the third variant, we provide constant numbers in the range $[0,1]$ as node features instead of using Deepwalk embeddings.

\begin{figure}[h]
    \centering
    \begin{subfigure}{.25\textwidth}
      \centering
      \includegraphics[width=\linewidth]{Images/Ablation/Rural.png}
    \end{subfigure}%
    \begin{subfigure}{.25\textwidth}
      \centering
      \includegraphics[width=\linewidth]{Images/Ablation/Animals.png}
    \end{subfigure}
    \begin{subfigure}{.25\textwidth}
      \centering
      \includegraphics[width=\linewidth]{Images/Ablation/rt.png}
    \end{subfigure}%
    \begin{subfigure}{.25\textwidth}
      \centering
      \includegraphics[width=\linewidth]{Images/Ablation/aids.png}
    \end{subfigure}
   \caption{Reward curves for variants of models with one of the component discussed in Section \ref{sec:abl} removed}
   \label{fig:abl}
\end{figure}


We show the reward curves in figure \ref{fig:abl} for three of our experiments where we trained on all of the training networks for each network family.
We note that in most cases the reward curve doesn't increase for architectures except our model. We conclude that in most settings all three components are vital to learning a stable policy.

